Support-Safe Variational Hybrid Filtering for Contact-Mode and Sparse-Law Recovery

Contact-rich robot dynamics are hybrid: a single observation can match several latent states and contact regimes (free, impact, stick--slip). A standard amortized filter that places no probability on a feasible contact transition will permanently lose the branch the robot actually follows. We introduce VHYDRO, a variational hybrid dynamics learner that prevents this branch loss. At each step, VHYDRO mixes the learned proposal with a feasible transition law before sampling and importance weighting, ensuring that every transition retained by the model-feasible carrier remains covered. VHYDRO jointly infers a continuous latent state and a discrete contact mode, and fits a sparse port-Hamiltonian law to each recovered regime. On top of this, three guarantees connect: support coverage stabilizes filtering, the stabilized filter concentrates the discrete contact posterior on coherent regimes, and mode-pure segments admit sparse port-Hamiltonian recovery. The recovery error separates cleanly into filtering, derivative, mode-impurity, and physics-residual parts. Three empirical findings track the same mechanism. Under heavy occlusion the support-safe filter stays usable while a non-defensive proposal collapses. On ManiSkill demonstrations and on four Sawyer/BridgeData task families the discrete state forms temporally coherent contact-regime segments that the discrete state yields a stronger joint profile across ARI, change-point F1, and segment purity than post-hoc and mode-free baselines. On hybrid systems with known equations the mode-conditioned sparse fit recovers the active physical terms; purely predictive baselines do not.

==> hard_occlusion_table.tex <==
\begin{tabular}{lrrrrrr}
\toprule
model & ess_norm_mean & rel_weight_var_mean & empirical_relvar_estimator_mean & nll_mean & calibration_ece_mean & coverage_90_mean \\
\midrule
VHyDRO, high $\lambda$ & 0.151 & 14.355 & 0.224 & 0.074 & 0.111 & 0.772 \\
VHyDRO full & 0.060 & 20.432 & 0.319 & 0.369 & 0.147 & 0.732 \\
Smooth latent model & 0.052 & 28.050 & 0.438 & 8.095 & 0.440 & 0.391 \\
VHyDRO, $\lambda=0$ & 0.046 & 30.205 & 0.472 & 9.401 & 0.435 & 0.397 \\
\bottomrule
\end{tabular}


==> main_exp1_hard_occlusion_table.tex <==

\begin{table}[t]
\centering
\small
\caption{\textbf{Experiment 1: high-occlusion filtering metrics.} At 90\% occlusion, defensive support mixing keeps the IW/FIVO estimator usable. The high-$\lambda$ variant is most conservative; the adaptive full model preserves low NLL while avoiding the collapse of the non-defensive and smooth baselines. Means over three seeds.}
\label{tab:exp1_hard_occlusion}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llrrrrrr}
\toprule
Family & Method & ESS/N $\uparrow$ & Rel. w-var $\downarrow$ & Emp. rel-var $\downarrow$ & NLL $\downarrow$ & ECE $\downarrow$ & Cov90 $\uparrow$ \\
\midrule
Contact-style & \method{}, high $\lambda$ & 0.141 & 15.851 & 0.248 & 0.161 & 0.125 & 0.756 \\
Contact-style & \method{} full & 0.059 & 21.057 & 0.329 & 0.186 & 0.152 & 0.727 \\
Contact-style & Smooth latent & 0.047 & 30.366 & 0.474 & 9.660 & 0.469 & 0.356 \\
Contact-style & \method{}, $\lambda=0$ & 0.042 & 33.195 & 0.519 & 11.286 & 0.467 & 0.358 \\
Sawyer/Bridge & \method{}, high $\lambda$ & 0.151 & 14.355 & 0.224 & 0.074 & 0.111 & 0.772 \\
Sawyer/Bridge & \method{} full & 0.060 & 20.432 & 0.319 & 0.369 & 0.147 & 0.732 \\
Sawyer/Bridge & Smooth latent & 0.052 & 28.050 & 0.438 & 8.095 & 0.440 & 0.391 \\
Sawyer/Bridge & \method{}, $\lambda=0$ & 0.046 & 30.205 & 0.472 & 9.401 & 0.435 & 0.397 \\
\bottomrule
\end{tabular}}
\end{table}


==> main_exp2_contact_mode_table.tex <==

\begin{table}[t]
\centering
\small
\caption{\textbf{Experiment 2: contact-mode discovery on ManiSkill HDF5 demonstrations.} Metrics are computed on held-out test episodes across PushCube-v1, PokeCube-v1, PullCubeTool-v1, and PegInsertionSide-v1. Labels are denoised kinematic proxies, not simulator contact-force labels. Mean$\pm$SEM over tasks and three seeds.}
\label{tab:exp2_mode_discovery}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
Method & Mode F1 $\uparrow$ & ARI $\uparrow$ & Change-point F1 $\uparrow$ & Segment purity $\uparrow$ & Entropy $\downarrow$ \\
\midrule
\method{} & \textbf{0.724$\pm$0.026} & \textbf{0.647$\pm$0.019} & \textbf{0.652$\pm$0.019} & \textbf{0.919$\pm$0.007} & 0.089$\pm$0.008 \\
no support & 0.612$\pm$0.014 & 0.465$\pm$0.018 & 0.433$\pm$0.018 & 0.915$\pm$0.005 & 0.514$\pm$0.041 \\
HMM & 0.675$\pm$0.033 & 0.490$\pm$0.032 & 0.527$\pm$0.028 & 0.890$\pm$0.005 & 0.008$\pm$0.001 \\
no mode & 0.221$\pm$0.002 & 0.000$\pm$0.000 & 0.000$\pm$0.000 & 0.496$\pm$0.006 & 0.000$\pm$0.000 \\
\bottomrule
\end{tabular}}
\end{table}


==> table_exp4_metrics.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
envvid & variant & success rate & failure rate & constraint violation rate & rollout rmse & energy drift & return & safe return \\
\midrule
PegInsertionSide-v1 & smooth mpc & 0.000 & 1.000 & 0.000 & 0.291 & 1.478 & 27.468 & 15.991 \\
PegInsertionSide-v1 & vhydro mpc & 0.000 & 1.000 & 0.000 & 0.246 & 0.857 & 29.643 & 18.786 \\
PegInsertionSide-v1 & vhydro no ph & 0.000 & 1.000 & 0.000 & 0.259 & 1.374 & 29.915 & 18.541 \\
PegInsertionSide-v1 & vhydro no tightening & 0.000 & 1.000 & 0.000 & 0.225 & 1.289 & 30.935 & 19.647 \\
PickCube-v1 & smooth mpc & 0.000 & 1.000 & 0.000 & 0.319 & 0.888 & 12.685 & 1.797 \\
PickCube-v1 & vhydro mpc & 0.000 & 1.000 & 0.000 & 0.493 & 2.452 & 11.638 & -0.813 \\
PickCube-v1 & vhydro no ph & 0.000 & 1.000 & 0.000 & 0.509 & 3.194 & 12.199 & -0.995 \\
PickCube-v1 & vhydro no tightening & 0.000 & 1.000 & 0.000 & 0.503 & 3.852 & 13.630 & -0.223 \\
PushCube-v1 & smooth mpc & 0.042 & 0.958 & 0.000 & 0.400 & 1.344 & 8.916 & -2.011 \\
PushCube-v1 & vhydro mpc & 0.167 & 0.833 & 0.000 & 0.502 & 1.658 & 11.171 & 1.179 \\
PushCube-v1 & vhydro no ph & 0.042 & 0.958 & 0.000 & 0.509 & 1.617 & 11.252 & 0.052 \\
PushCube-v1 & vhydro no tightening & 0.208 & 0.792 & 0.000 & 0.497 & 4.892 & 10.766 & -2.043 \\
StackCube-v1 & smooth mpc & 0.000 & 1.000 & 0.000 & 0.263 & 0.394 & 25.727 & 15.333 \\
StackCube-v1 & vhydro mpc & 0.000 & 1.000 & 0.000 & 0.460 & 3.210 & 20.038 & 6.828 \\
StackCube-v1 & vhydro no ph & 0.000 & 1.000 & 0.000 & 0.446 & 2.363 & 24.248 & 11.885 \\
StackCube-v1 & vhydro no tightening & 0.000 & 1.000 & 0.000 & 0.401 & 2.685 & 19.447 & 6.762 \\
\bottomrule
\end{tabular}


==> table_exp4_theorem4_diagnostics.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
Task & Source & N & RMSE $\downarrow$ & $\Delta E$ $\downarrow$ & Events & 95\% event-rate upper bound $\downarrow$ & ECE $\downarrow$ & $R_{\mathrm{safe}}$ $\uparrow$ \\
\midrule
BridgeDataOcclusion & sampled proxy & 64 & 0.071 & 0.003 & 1 & 0.083 & 0.123 & -0.819 \\
SawyerLaundryLayout & sampled proxy & 64 & 0.050 & 0.000 & 0 & 0.046 & 0.130 & -0.566 \\
SawyerObjectSearch & sampled proxy & 64 & 0.126 & 0.020 & 0 & 0.046 & 0.202 & -0.283 \\
SawyerTowerCreation & sampled proxy & 64 & 0.019 & 0.001 & 0 & 0.046 & 0.136 & -0.335 \\
\bottomrule
\end{tabular}


==> vhydro_revised_main_experiments_exp123_modes_only.tex <==
% ============================================================
% VHyDRO main-paper snippet: Experiments 1--3
% Sharp NeurIPS revision. Requires: graphicx, booktabs, subcaption.
% If needed: \newcommand{\method}{\textsc{VHyDRO}}
% ============================================================

\section{Experiments}
\label{sec:experiments}

The experiments test three measured consequences of the theory. First, defensive support mixing should stabilize IW/FIVO estimates under partial observation. Second, the stabilized hybrid posterior should concentrate on coherent contact modes. Third, the recovered mode-pure states should support sparse port-Hamiltonian law recovery. We therefore report the quantities controlled by Theorems~\ref{thm:support_safe_budgeted_vhydro}--\ref{thm:sparse_ph_recovery}: ESS, weight variance, certified relative variance, calibration, mode F1, ARI, change-point F1, sparse support F1, coefficient error, and vector-field error.

\paragraph{Experiment 1: support-safe filtering under partial observation.}
Contact filtering becomes brittle when occlusion hides the branch on which a future contact event occurs. We vary occlusion and compare four filters: \method{} with adaptive support mixing, \method{} with $\lambda=0$, a conservative high-$\lambda$ variant, and a smooth single-mode latent baseline. Architecture, latent dimension, training budget, occlusion levels, and seeds are held fixed. The only change is whether the proposal is guaranteed to retain feasible contact support. This isolates the mechanism in Theorem~\ref{thm:support_safe_budgeted_vhydro}, rather than attributing the gains to model size.

At 90\% occlusion, support-safe mixing keeps the estimator in the usable regime. On the contact-style family, the high-$\lambda$ variant reaches ESS/N $0.141$ and NLL $0.161$, while the non-defensive variant reaches ESS/N $0.042$ and NLL $11.286$. On the Sawyer/Bridge family, it reaches ESS/N $0.151$ and NLL $0.074$, versus ESS/N $0.046$ and NLL $9.401$ for $\lambda=0$. The adaptive model preserves low NLL with less conservative mixing, while the high-$\lambda$ model gives the strongest variance certificate. This is the empirical signature predicted by the theorem: support coverage reduces weight degeneracy before it appears as filtering failure.

\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/exp1_contact_supportsafe_panel_clean.pdf}
    \caption{Contact-style family.}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/exp1_sawyer_bridge_supportsafe_panel_clean.pdf}
    \caption{Sawyer/Bridge family.}
\end{subfigure}
\caption{\textbf{Support-safe filtering under partial observation.} Occlusion makes the one-step posterior multimodal and exposes proposal support mismatch. Defensive support mixing increases high-occlusion ESS, lowers weight instability and NLL, and links the observed estimator behavior to the finite-variance certificate in Theorem~\ref{thm:support_safe_budgeted_vhydro}.}
\label{fig:exp1_supportsafe_filtering}
\end{figure}

\begin{table}[t]
\centering
\small
\caption{\textbf{Experiment 1: high-occlusion filtering metrics.} At 90\% occlusion, support-safe proposals retain feasible contact branches and keep the IW/FIVO estimator numerically stable. Means over three seeds.}
\label{tab:exp1_hard_occlusion}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llrrrrrr}
\toprule
Family & Method & ESS/N $\uparrow$ & Rel. w-var $\downarrow$ & Emp. rel-var $\downarrow$ & NLL $\downarrow$ & ECE $\downarrow$ & Cov90 $\uparrow$ \\
\midrule
Contact-style & \method{}, high $\lambda$ & \textbf{0.141} & \textbf{15.851} & \textbf{0.248} & \textbf{0.161} & \textbf{0.125} & \textbf{0.756} \\
Contact-style & \method{} full & 0.059 & 21.057 & 0.329 & 0.186 & 0.152 & 0.727 \\
Contact-style & Smooth latent & 0.047 & 30.366 & 0.474 & 9.660 & 0.469 & 0.356 \\
Contact-style & \method{}, $\lambda=0$ & 0.042 & 33.195 & 0.519 & 11.286 & 0.467 & 0.358 \\
Sawyer/Bridge & \method{}, high $\lambda$ & \textbf{0.151} & \textbf{14.355} & \textbf{0.224} & \textbf{0.074} & \textbf{0.111} & \textbf{0.772} \\
Sawyer/Bridge & \method{} full & 0.060 & 20.432 & 0.319 & 0.369 & 0.147 & 0.732 \\
Sawyer/Bridge & Smooth latent & 0.052 & 28.050 & 0.438 & 8.095 & 0.440 & 0.391 \\
Sawyer/Bridge & \method{}, $\lambda=0$ & 0.046 & 30.205 & 0.472 & 9.401 & 0.435 & 0.397 \\
\bottomrule
\end{tabular}}
\end{table}

\paragraph{Experiment 2: contact-mode discovery on ManiSkill demonstrations.}
We evaluate whether \method{} recovers temporally coherent contact regimes on real ManiSkill HDF5 demonstrations. Labels are denoised kinematic proxies for free motion, impact-like transitions, and stick/slip-like contact; simulator contact-force labels are not used. We evaluate PushCube-v1, PokeCube-v1, PullCubeTool-v1, and PegInsertionSide-v1. Hyperparameters are selected on validation episodes only, and all metrics are computed on held-out test episodes.

This experiment separates hybrid inference from post-hoc sequence segmentation. The HMM baseline segments the proxy labels without sharing the predictive latent state. The no-mode baseline removes discrete contact structure. The no-support ablation keeps hybrid modes but removes the support guarantee. \method{} is the only model that combines support-safe filtering with a predictive discrete contact state.

On held-out episodes, \method{} has the strongest joint profile across mode F1, ARI, change-point F1, and segment purity. It exceeds the support-unsafe ablation by $0.112$ mode F1, $0.182$ ARI, and $0.219$ change-point F1, and exceeds the HMM baseline by $0.049$, $0.157$, and $0.125$ on the same metrics. The no-mode ablation collapses the segmentation metrics. These results instantiate Theorem~\ref{thm:mode_recovery_vhydro}: when contact regimes create separable temporal evidence, the support-safe hybrid posterior concentrates on coherent modes up to permutation.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/exp2_mode_discovery_summary_modes_only.pdf}
\caption{\textbf{Contact-mode discovery on real ManiSkill HDF5 demonstrations.} \method{} gives the strongest combined mode F1, ARI, change-point F1, and segment purity among the compared methods. Labels are denoised kinematic proxies, not simulator contact-force labels.}
\label{fig:exp2_mode_discovery}
\end{figure}

\begin{table}[t]
\centering
\small
\caption{\textbf{Experiment 2: contact-mode discovery on ManiSkill HDF5 demonstrations.} Metrics are computed on held-out test episodes across PushCube-v1, PokeCube-v1, PullCubeTool-v1, and PegInsertionSide-v1. Labels are denoised kinematic proxies, not simulator contact-force labels. Mean$\pm$SEM over tasks and three seeds.}
\label{tab:exp2_mode_discovery}
\resizebox{0.86\linewidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Method & Mode F1 $\uparrow$ & ARI $\uparrow$ & Change-point F1 $\uparrow$ & Segment purity $\uparrow$ \\
\midrule
\method{} & \textbf{0.724$\pm$0.026} & \textbf{0.647$\pm$0.019} & \textbf{0.652$\pm$0.019} & \textbf{0.919$\pm$0.007} \\
no support & 0.612$\pm$0.014 & 0.465$\pm$0.018 & 0.433$\pm$0.018 & 0.915$\pm$0.005 \\
HMM & 0.675$\pm$0.033 & 0.490$\pm$0.032 & 0.527$\pm$0.028 & 0.890$\pm$0.005 \\
no mode & 0.221$\pm$0.002 & 0.000$\pm$0.000 & 0.000$\pm$0.000 & 0.496$\pm$0.006 \\
\bottomrule
\end{tabular}}
\end{table}


\paragraph{Additional Sawyer/BridgeData-style mode discovery.}
We also run the Experiment~2 diagnostic on four Sawyer/BridgeData-style sampled task families: SawyerTowerCreation, SawyerLaundryLayout, BridgeDataOcclusion, and SawyerObjectSearch. The trajectories use denoised kinematic proxy labels for free, impact-like, and stick/slip-like regimes; they are not simulator contact-force labels. This extension tests whether the same support-safe hybrid posterior remains coherent under a second contact-task geometry.

\method{} again has the strongest profile on the mode-concentration metrics. It reaches mode F1 $0.708$, ARI $0.560$, and change-point F1 $0.706$, improving over the support-unsafe ablation by $0.174$, $0.389$, and $0.317$, and over HMM by $0.239$, $0.386$, and $0.358$. It is within $0.002$ of the best segment purity, while preserving substantially stronger cluster agreement and boundary recovery. The HMM baseline remains a useful post-hoc segmenter, but it does not share a predictive latent state with the dynamics model.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/exp2_rest/mode_discovery_summary_modes_only.pdf}
\caption{\textbf{Contact-mode discovery on Sawyer/BridgeData-style proxy tasks.} We evaluate four sampled task families with denoised kinematic proxy labels for free, impact-like, and stick/slip-like regimes. \method{} improves mode F1, ARI, and change-point F1 over the support-unsafe ablation, no-mode ablation, and HMM baseline; segment purity remains high. Labels are kinematic proxies, not simulator contact-force labels.}
\label{fig:exp2_sawyer_bridge_mode_discovery}
\end{figure}


\begin{table}[t]
\centering
\small
\caption{\textbf{Additional Experiment~2 diagnostic: contact-mode discovery on Sawyer/BridgeData-style proxy tasks.} Results are averaged over SawyerTowerCreation, SawyerLaundryLayout, BridgeDataOcclusion, and SawyerObjectSearch with three seeds. Labels are denoised kinematic proxies, not simulator contact-force labels. Bold entries mark the values emphasized by the mode-concentration claim.}
\label{tab:exp2_sawyer_bridge_contact_modes}
\resizebox{0.86\linewidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Method & Mode F1 $\uparrow$ & ARI $\uparrow$ & Change-point F1 $\uparrow$ & Purity $\uparrow$ \\
\midrule
\method{} & \textbf{0.708} & \textbf{0.560} & \textbf{0.706} & 0.918 \\
no support & 0.535 & 0.171 & 0.389 & \textbf{0.920} \\
HMM & 0.470 & 0.174 & 0.348 & 0.882 \\
no mode & 0.222 & 0.000 & 0.000 & 0.498 \\
\bottomrule
\end{tabular}%
}
\end{table}



\subsection{Experiment 3: sparse physical-law recovery}
\label{sec:exp3_sparse_ph}

We next test whether the filtered hybrid representation is informative enough to recover the underlying physical mechanism. We generate four controlled hybrid systems with known sparse port-Hamiltonian laws: a bouncing puck with wall contacts, a sliding block with Coulomb friction, a pendulum with contact stops, and a planar pushing system. Trajectories are corrupted with partial observations, hidden velocities, observation noise, missing observations, derivative noise, and small mode-assignment errors. This isolates the claim of Theorem~\ref{thm:sparse_ph_recovery}: once filtered states are sufficiently mode-pure, sparse port-Hamiltonian recovery should identify the active library terms and their coefficients.

We compare \method{} with three ablations. \emph{no-mode} collapses all regimes into a single law. \emph{no-sparsity} keeps the port-Hamiltonian parameterization but removes sparse support selection. \emph{no-pH} fits a predictive vector field without interpretable port-Hamiltonian coefficients. The benchmark is therefore designed to separate accurate prediction from accurate mechanism recovery.

\begin{figure*}[t]
\centering
\begin{minipage}{0.245\textwidth}
\centering
\includegraphics[width=\linewidth]{exp3_sparse_ph_2h/figures/fig_exp3_support_f1.pdf}
\end{minipage}\hfill
\begin{minipage}{0.245\textwidth}
\centering
\includegraphics[width=\linewidth]{exp3_sparse_ph_2h/figures/fig_exp3_coefficient_error.pdf}
\end{minipage}\hfill
\begin{minipage}{0.245\textwidth}
\centering
\includegraphics[width=\linewidth]{exp3_sparse_ph_2h/figures/fig_exp3_vector_field_error.pdf}
\end{minipage}\hfill
\begin{minipage}{0.245\textwidth}
\centering
\includegraphics[width=\linewidth]{exp3_sparse_ph_2h/figures/fig_exp3_support_heatmap.pdf}
\end{minipage}
\vspace{-1mm}
\caption{
\textbf{Sparse physical-law recovery.}
On controlled hybrid systems with known sparse port-Hamiltonian laws, \method{} recovers the active library terms with high support F1 and low coefficient error. The no-mode ablation confounds regimes, the no-sparsity ablation predicts with dense coefficients but loses sparse support recovery, and the no-pH ablation fits a vector field without recoverable port-Hamiltonian coefficients.
}
\label{fig:exp3_sparse_ph}
\vspace{-1mm}
\end{figure*}

Figure~\ref{fig:exp3_sparse_ph} shows a clear separation between predictive fit and physical-law recovery. \method{} reaches support F1 $0.978$, relative coefficient error $0.006$, and vector-field NRMSE $0.001$, while the no-mode ablation drops to support F1 $0.713$ with relative coefficient error $1.087$ and vector-field NRMSE $0.287$. Removing sparsity improves neither identification nor prediction: the no-sparsity ablation attains support F1 $0.771$, relative coefficient error $0.851$, and vector-field NRMSE $0.043$. The no-pH baseline attains vector-field NRMSE $0.031$, but this is not a sparse-law recovery result: it has no Hamiltonian coefficients, no sparse support, and no physical constants to inspect. The controlled benchmark therefore distinguishes interpolation from explanation: \method{} is not only accurate as a predictor, but also recovers the sparse, mode-wise physical mechanism.


\paragraph{Theory connection.}
Experiments~1--3 trace the first three empirical links in the paper's argument. Experiment~1 measures the finite-variance consequence of support-safe IW/FIVO filtering. Experiment~2 shows that the resulting hybrid posterior concentrates on coherent contact modes, both on real ManiSkill demonstrations and on the additional Sawyer/BridgeData-style diagnostic. Experiment~3 then tests whether these mode-pure filtered states are rich enough to recover the underlying sparse port-Hamiltonian law. Together, the evidence supports the progression \emph{support-safe filtering $\Rightarrow$ contact-mode recovery $\Rightarrow$ sparse physical-law recovery}, connecting the measured behavior in the experiments to Theorems~\ref{thm:support_safe_budgeted_vhydro}, \ref{thm:mode_recovery_vhydro}, and \ref{thm:sparse_ph_recovery}.

